NAIST-SIC-Aligned: an Aligned English-Japanese Simultaneous Interpretation Corpus

It remains a question that how simultaneous interpretation (SI) data affects simultaneous machine translation (SiMT). Research has been limited due to the lack of a large-scale training corpus. In this work, we aim to fill in the gap by introducing NAIST-SIC-Aligned, which is an automatically-aligned parallel English-Japanese SI dataset. Starting with a non-aligned corpus NAIST-SIC, we propose a two-stage alignment approach to make the corpus parallel and thus suitable for model training. The first stage is coarse alignment where we perform a many-to-many mapping between source and target sentences, and the second stage is fine-grained alignment where we perform intra- and inter-sentence filtering to improve the quality of aligned pairs. To ensure the quality of the corpus, each step has been validated either quantitatively or qualitatively. This is the first open-sourced large-scale parallel SI dataset in the literature. We also manually curated a small test set for evaluation purposes. Our results show that models trained with SI data lead to significant improvement in translation quality and latency over baselines. We hope our work advances research on SI corpora construction and SiMT. Our data can be found at https://github.com/mingzi151/AHC-SI.

==> sections/2-0-related-work.tex <==

\section{Related work}

\subsection{Simultaneous interpretation}
%  what I want to express in this section: 1) SI is different; interpreters use strategies. The nature of SI makes online data different from offline data. Despite this, cognitive load leads to errors in the outputs. 

Simultaneous interpretation (SI)  demands a great deal of cognitive load, which makes the task challenging for interpreters \citep{mizuno2017simultaneous}. It is of essence that interpreters use strategies to minimize delay and reduce the load of retention \citep{mizuno2017simultaneous,DBLP:conf/naacl/HeBD16, dong2019acquisition}. 
% Previous works in various disciplines (e.g., translation and interpreting studies, and NLP) have grouped these strategies from different perspectives. 
% One example of the strategies is \textit{segmentation} where interpreters break a source sentence into several smaller chucks and interpret by chunks \citep{camayd2011cognitive}. %\mich{(Need help from Doi-san: can you please find me such an example)}
% ii) \textbf{Generalization} when interpreters give up original source words and restate the source message in their own ways \citep{camayd2011cognitive}. 
% Another one 
Examples of these strategies include \textit{summarisation} where interpreters omit unimportant words or condense contents to simplify overwhelming information,
% For example, "in the last years of the old regime" can be condensed into "\jap{昔は}" (in the past) in an SI sentence and literately translated into "\jap{旧体制の終わりの時期には}" (At the end of the old system) in the offline translation. 
and \textit{segmentation} where interpreters break a source sentence into several smaller chunks and interpret by chunks \citep{camayd2011cognitive}. Other strategies include \textit{generalization} when interpreters give up original source words and restate the source message in their own ways \citep{camayd2011cognitive}.
% , and \textit{passivization} \citep{DBLP:conf/emnlp/HeGMBD15} when interpreters use passive voices and drop subjects to avoid waiting for verbs.

These tactics make interpreted texts inherently different from translated texts where heavy post-editing (e.g., reordering, use of sophisticated vocabulary) is involved.

% Despite of the strategies, cognitive load leads to erroneous outputs~\cite{zhao2021not}. 
%\mich{(Need help from Doi-san: can you please find me such an example)}
% \mich{Examples of them are shown in Table~\ref{tab:strategy-example}.}
% iv) \textbf{Passivization} \citep{DBLP:conf/emnlp/HeGMBD15} when interpreters use passive voices and drop subjects to avoid waiting for verbs.
% , which is particularly helpful to interpret sources in SOV languages (e.g., Japanses) to target SVO languages (e.g., English). 
% Table \ref{tab:strategies} provides illustrations of above stratgies.
% The adopted tactics make interpreted texts inherently different from translated texts. Yet since , 
% Hence, learning human interpretation data directly could result in suboptimal solutions~\cite{shimizu2013constructing}. 
% SI corpus construction requires great efforts and care. 
% Therefore, SI corpus construction requires great efforts and care. 

% However, very little attempt has been made on creating datasets or evaluation benchmarks that reflect on these well-documented differences. 


\begin{comment}
\begin{table*}[!t]
\centering
\small
  \scalebox{0.95}
  {
  \begin{tabular}{p{2cm}|p{4.2cm}|p{4.2cm}|p{4.2cm}}
    \toprule
    \textbf{Strategy} & \textbf{Source} & \textbf{Interpreted Text} & \textbf{Translated Text}  \\
    \midrule
    Segmentation \textcolor{red}{|||} & And I claim it's already today that it's more likely for any of us to become the victim of a crime online than here in the real world. & \jap{\scriptsize 私は今日、主張したいと思います、} \textcolor{red}{|||} \jap{\scriptsize 今おそらく、このようなオンライン犯罪の、犠牲者になりうるというわけなんです、} \textcolor{red}{|||} \jap{\scriptsize 現実の世界よりも、可能性は高いんです。} & \jap{\scriptsize 今日の時点ですでに、リアルの世界で犯罪に遭うより、オンライン犯罪の被害者になる可能性の方が、高いのではと考えています。} \\
     & & {\footnotesize [I claim today \textcolor{red}{|||} it's likely to become the victim of a crime online \textcolor{red}{|||} more likely than in the real world]} & \\
    Summarization & And {\color{blue}in the last years of the old regime,} he would routinely be detailed to go into the township to aggress the community. & \jap{\scriptsize \textcolor{blue}{昔は、}} \textcolor{blue}{[in the past]} \jap{\scriptsize 警察と言うのが、タウンシップに行って、コミュニティの攻撃していた訳です。} & \jap{\scriptsize \textcolor{blue}{旧体制の終わりの時期には、}非白人居住区の人々への攻撃に、たびたび派遣されていました。} \\
    \bottomrule
  \end{tabular}
  }

  \caption{Examples of strategies used by simultaneous interpreters}
  \label{tab:strategy-example}
\end{table*}
\end{comment}

\subsection{Simultaneous Interpretation Corpus}
% \todo{Doi-san: can you please continue from here? In the first paragraph, you will list popular SI data. In addition to what you covered in your paper, please also do a bit more literature review and cover other datasets that are published after your work. To name a few, my paper, 
% VoxPopuli data (published by Meta). Please use a table to report data statistics. Then in the second paragraph, please briefly explain why alignment is difficult. Write ~1/2 column}. 
Current publicly available SI corpora have remained limited in size (see Table~\ref{tab:corpora-list}\footnote{The pSp corpus introduced in~\citet{Paulik-and-Waibel-2009} replies heavily on time information. Its quality is unclear due to the lack of open-source accessibility.}), and most of them can only be used for evaluation.
This is because SI corpus construction demands immense effort and care.
Converting interpreters' speech to text would involve post-editing on ASR outputs.
More importantly, aligning sentences of parallel SI documents, either manually or automatically, exhibits great challenges due to the nature of SI.
% First, converting interpreters' speech to text would involve post-editing on ASR outputs.
% ; ASR errors can lead to low-quality alignments. 
% More importantly, 
The cognitive load of interpreters leads to erroneous outputs~\cite{Paulik-and-Waibel-2009,zhao2021not}, which would require filtering in alignment.
For instance, interpreters may unintentionally omit important content, and one would need to identify this phenomenon and apply filtering accordingly.
Additional filtering might also be required when interpreters intentionally omit content to facilitate the service~\cite{DBLP:conf/naacl/HeBD16}. 

Furthermore, unlike in offline MT, source and target sentences in SI may not necessarily follow one-to-one relationship.
For example, interpreters may summarise a number of source sentences into one target sentence or break a long source sentence into a few target sentences.
In these cases, practitioners or annotators need to recognise them correctly and perform sentence merging.
The unique characteristics of SI make SI corpus alignment a difficult task, even for human annotators. 

In this work, starting from conducting error analysis on the corpus proposed in~\cite{doi2021large}, we design a language-agnostic alignment approach to build a training corpus for SiMT. We expect our approach to be extendable to other language pairs.  
% Consequently,  
% In the 2020s, several datasets were released one after another, some of which are relatively large-scale. 

% Another challenge to construct SI corpora is related to alignment. Manual alignment is costly and time-consuming, while automated methods, such as those yielded by ASR~\cite{wang-etal-2021-voxpopuli}, require careful filtering because ASR errors can lead to low-quality alignments.

% In addition, the characteristics of SI make the alignments difficult. For example, source and target texts do not necessarily match due to omission, summarisation, or mis-translation. In another case, multiple sentences can be interpreted into one sentence. Because of these unique features of SI text, SI corpus alignment is a difficult task even for human annotators.

\begin{table}
\centering
\small
% \scalebox{0.9}
\scalebox{0.85}{
\begin{tabular}{lcc}
\hline \textbf{Corpora} & \textbf{Language} & \textbf{Size} \\
\hline
\citet{Tohyama-et-al-2004} & En$\leftrightarrow$Jp & 182 hours \\
\citet{shimizu2014collection} & En$\leftrightarrow$Jp & 22 hours \\
\citet{doi2021large} & En$\leftrightarrow$Jp & 304.5 hours \\
\hline
\citet{pan2019chinese} & Zh$\leftrightarrow$En & 6M tokens \\
\citet{zhang2021bstc}~(dev/test) & Zh$\rightarrow$En & 3 hours  \\
\hline
\citet{Paulik-and-Waibel-2009} & En$\leftrightarrow$Es & 217 hours \\
\citet{bernardini2016epic} & En, Fr, It & 95K tokens \\
\citet{kunz2021heicic} & En$\leftrightarrow$De & 83 hours \\
\citet{zhao2021not} & En$\leftrightarrow$De & 1K sent. \\
\citet{machacek21_interspeech} & En$\rightarrow$De, Cs & 10 hours \\
\citet{wang2021voxpopuli} & 15 lang. & 17.3K hours \\
\citet{przybyl2022epic} & En, De, Es & 10K sent. \\
\hline
\end{tabular}}
\caption{Existing SI corpora.}
\label{tab:corpora-list}
\end{table}

\begin{comment}
\subsection{Simultaneous machine translation}
% \todo{ToDo by Ryo-san: in a first paragraph, start with the overall development of SiMT. then focus on describing wait-k and mention we use it throughtout our work. Then in a second paragraph, say these models are all trained on offline MT data, point out the potential problems and highlight the gap that we try to fill in  in this work.Write ~1/2 column}
Early attempts on SiMT include rule-based machine translation \cite{matsubara1997incremental} and statistical methods using statistical machine translation \cite{bangalore-etal-2012-real}. Recent studies have applied neural machine translation (NMT) to SiMT \cite{gu-etal-2017-learning,arivazhagan-etal-2019-monotonic, elbayad20_interspeech}.
One remarkable work is \citet{ma-etal-2019-stacl} where the authors presented a wait-k policy that first waits for k source words and then translates the rest of the source sentences simultaneously, and they trained RNN or Transformer  \cite{vaswani2017attention} using the wait-k policy.
This deterministic approach gained great popularity because of its simplicity and effectiveness. 
% is still popular today because it is simple but effective.
Throughout our work, we use Transformer-based wait-k models as our SiMT systems.

SiMT differs from offline MT by nature, but most SiMT systems are trained on offline translation corpora due to a lack of a large, high-quality SI corpus.
This is far from ideal for the simultaneous scenario, as there is a lot of unnecessary long-distance reordering in these corpora \cite{chen-etal-2021-improving-simultaneous}.

% From early attempts using rule-based machine translation \cite{matsubara1997incremental,ryu-etal-2006-simultaneous} and statistical methods using statistical machine translation \cite{bangalore-etal-2012-real,fujita-etal-2013-simple}, recent studies have successfully applied neural machine translation (NMT) to SiMT \cite{gu-etal-2017-learning,ma-etal-2019-stacl,arivazhagan-etal-2019-monotonic, elbayad20_interspeech}.
% \citet{ma-etal-2019-stacl} presented a wait-k policy that first waits for k source words and then translates the rest of the source sentences simultaneously, and they trained RNN or Transformer  \cite{vaswani2017attention} using the wait-k policy.
% This deterministic approach is still popular today because it is simple but effective.
% Throughout our work, we focus on the Transformer-based wait-k model as SiMT.

% Although SiMT is a very different task from offline MT, most SiMT systems are trained on offline translation corpora due to lacking a large, high-quality SI corpus.
% This is far from ideal for the simultaneous scenario, as there is a lot of unnecessary long-distance reordering in these corpora \cite{chen-etal-2021-improving-simultaneous}.


\mich{~3 pages in total up to here}
\end{comment}

==> sections/4-results.tex <==
\section{Results} \label{results}





% \subsection{Main results (Data selection)}

% As mentioned in \S\ref{coarse} (Finding), the quality of SI data varies by talk and thus the quality of the aligned pairs, so we investigate the impact of data quality on model performance. We select subsets of the corpus from the following perspectives. i) \textit{Interpreter rank}: S-ranked interpreters who are more experienced than A-ranked interpreters tend to have better interpreting performance. ii) \textit{Speaker speed}: it is assumed that fast-speaking speakers would make it challenging for the interpreter to understand and interpret the content. iii) Content coverage: our hypothesise is that the more content covered by an SI sentence, the better quality of the pair is. We measure content coverage with the criteria set in \S\ref{fine} (Inter-sentence filtering). We also consider different combinations of the above data selection strategies. 

% % \paragraph{Interpreter rank}


% % \paragraph{Speaker speed}

% \subsection{Subjective evaluation}
% which is the best model

% which metric works the best.  

% % \paragraph{Content coverage}
% \subsection{BLEU vs BLEURT}
% Ideally, BLEURT should yield more reliable results than BLEU~\cite{freitag2022results}, particularly for the task of the concern that emphasise the semantic similarly rather than token-level similary. However, in our preliminary experiments, we find that BLEU and BLEURT give contradicting results as which model performs the best. To find out the correct metric to use, we employed three interpreters to conduct pairwise evaluation on the outputs of three models. We found XXXX.

% \subsection{Punctuation removal}
% We notice that the outputs of SiMT trained with SI data contain commas more than necessary. 
% % This is expected, as we join SI chunks with commas to indicate where interpreters take 

% \subsection{Latency regime}
% \mich{Should we discuss this as well? Recall that models trained with SI data in the mid/high latency regimes hurt translation and latency}



% \subsection{Offline test set}
% For completeness, we also reported results on offline data which consist of pairs <source, translation>. The test set is constructed the same way described in the coarse alignment section and no further editing is required. Overall, XXX. We provide detailed results in Appendix XX.






